OVANet: One-vs-All Network for Universal Domain Adaptation

Universal Domain Adaptation (UNDA) aims to handle both domain-shift and category-shift between two datasets, where the main challenge is to transfer knowledge while rejecting unknown classes which are absent in the labeled source data but present in the unlabeled target data. Existing methods manually set a threshold to reject unknown samples based on validation or a pre-defined ratio of unknown samples, but this strategy is not practical. In this paper, we propose a method to learn the threshold using source samples and to adapt it to the target domain. Our idea is that a minimum inter-class distance in the source domain should be a good threshold to decide between known or unknown in the target. To learn the inter-and intra-class distance, we propose to train a one-vs-all classifier for each class using labeled source data. Then, we adapt the open-set classifier to the target domain by minimizing class entropy. The resulting framework is the simplest of all baselines of UNDA and is insensitive to the value of a hyper-parameter yet outperforms baselines with a large margin.

==> LaTeX/tables/anomaly_supple.tex <==
\begin{table*}[ht]
\begin{center}
 %\addtolength{\tabcolsep}{-3pt}

\begin{tabular}{@{}c|c|cccc@{}}

\toprule[1.5pt]
$\mathcal{D}_{\text{in}}$ & $\mathcal{D}_{\text{out}}$  &Acc &UNK&H-Score / Best &Overall Acc / Best\\ \midrule
%\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\small CIFAR-10}}} 
\multirow{2}{*}{CIFAR-10} & CIFAR-100      &91.9 &67.1&77.5 / 85.3&79.5 / 85.5\\
 & SVHN            &91.9 &84.6&88.1 / 91.3&86.7 / 93.8 \\
\midrule
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\small CIFAR-100 80}}}
\multirow{3}{*}{CIFAR-100-80} & CIFAR-100-20       & 94.8 &63.1& 64.3 /  64.7 & 64.3 / 65.4\\
 & CIFAR-10        &94.8 & 69.0	& 67.2 / 67.3& 67.3 / 68.0\\
 & SVHN            & 94.8 & 74.5&69.7 / 69.8	& 72.0 / 80.9\\
 \bottomrule[1.5pt]
\end{tabular}
\caption{\textbf{Results in open-set recognition.} Acc shows the accuracy to accept the in-lier samples as known, UNK denotes the accuracy to reject the out-lier dataset as unknown. H-score considers the trade-off between Acc and UNK. \ours performs comparable well to \textit{Best} scores, which indicate that the decided threshold is close to the optimal one. }
\label{tab:anomay_csi}

\end{center}
\end{table*}


==> LaTeX/tables/cifar_open.tex <==
\begin{table}[t]
 \addtolength{\tabcolsep}{-3pt}
\begin{center}
\scalebox{0.9}{

\begin{tabular}{l|ccc|ccc}
\toprule[1.5pt]
\multirow{2}{*}{Threshold}& \multicolumn{3}{c|}{CIFAR100}& \multicolumn{3}{c}{CIFAR10}\\\
     & 50 / 50  & 70 / 30  & 80 / 20   & 5 / 5 & 7 / 3  & 8 / 2     \\\hline
     \rowcolor{Gray}
\ours &61.7&68.8&64.8&56.1&62.1&62.8\\ 
Grid Search&68.1&68.9&64.9&66.1&62.2&64.8\\ \hline
Difference & 6.4&0.1&0.1&10.0&0.1&2.0\\

  \bottomrule[1.5pt]

\end{tabular}}
\end{center}
\vspace{-7mm}
\caption{\small \textbf{Accuracy in open-set recognition}, where a model does not see any unlabeled samples during training. No. of known / unknown classes are shown in each column. }
\label{tb:cifar}
  \vspace{-2mm}
\end{table}

==> LaTeX/tables/office_obda.tex <==

\begin{table}[t]
 \addtolength{\tabcolsep}{-3pt}

\begin{center}
%The result of STA in a \kate{???}lower row is from reported results~\cite{Liu_2019_CVPR} and that of Office-Home and VisDA is obtained by optimizing hyper-parameters.}
\scalebox{0.95}{

\begin{tabular}{l|cccccc|c}
\toprule[1.5pt]
\multirow{2}{*}{Method}& \multicolumn{6}{c|}{Office(10 / 10 / 11)}&\\
& A2W	& D2W & W2D & A2D & D2A & W2A& Avg\\\cline{1-8}
UAN~\cite{UDA_2019_CVPR}  &\\
CMU~\cite{bucci2020effectiveness} & \\
DANCE~\cite{saito2020universal} & \\\hline
\rowcolor{Gray}
\ours w/o OEM & &&&&&&\\
\rowcolor{Gray}
\ours & &&&&&&\\
  \bottomrule[1.5pt]
\end{tabular}
}
\caption{\small Results on open-partial domain adaptation.}

\label{tb:office_opda}
\end{center}
\vspace{-5mm}
\end{table}


==> LaTeX/tables/office_opda.tex <==

\begin{table}[t]
 \addtolength{\tabcolsep}{-3pt}

\begin{center}
%The result of STA in a \kate{???}lower row is from reported results~\cite{Liu_2019_CVPR} and that of Office-Home and VisDA is obtained by optimizing hyper-parameters.}
\scalebox{0.95}{

\begin{tabular}{l|cccccc|c}
\toprule[1.5pt]
\multirow{2}{*}{Method}& \multicolumn{6}{c|}{Office(10 / 0 / 3, 6, 9, 11)}&\\
& A2W	& D2W & W2D & A2D & D2A & W2A& Avg\\\cline{1-8}
UAN~\cite{UDA_2019_CVPR}  &\\
%CMU~\cite{fu2020learning} &\\
ROS~\cite{bucci2020effectiveness} & \\
DANCE~\cite{saito2020universal} & \\\hline
\rowcolor{Gray}
So-OpenNet & &&&&&&\\
\rowcolor{Gray}
OpenNet & &&&&&&\\
  \bottomrule[1.5pt]
\end{tabular}
}
\caption{\small Results on open-set domain adaptation. }

\end{center}
\vspace{-5mm}
\end{table}

